Static and Animated 3D Scene Generation from Free-form Text Descriptions

Generating coherent and useful image/video scenes from a free-form textual description is technically a very difficult problem to handle. Textual description of the same scene can vary greatly from person to person, or sometimes even for the same person from time to time. As the choice of words and syntax vary while preparing a textual description, it is challenging for the system to reliably produce a consistently desirable output from different forms of language input. The prior works of scene generation have been mostly confined to rigorous sentence structures of text input which restrict the freedom of users to write description. In our work, we study a new pipeline that aims to generate static as well as animated 3D scenes from different types of free-form textual scene description without any major restriction. In particular, to keep our study practical and tractable, we focus on a small subspace of all possible 3D scenes, containing various combinations of cube, cylinder and sphere. We design a two-stage pipeline. In the first stage, we encode the free-form text using an encoder-decoder neural architecture. In the second stage, we generate a 3D scene based on the generated encoding. Our neural architecture exploits state-of-the-art language model as encoder to leverage rich contextual encoding and a new multi-head decoder to predict multiple features of an object in the scene simultaneously. For our experiments, we generate a large synthetic data-set which contains 13,00,000 and 14,00,000 samples of unique static and animated scene descriptions, respectively. We achieve 98.427% accuracy on test data set in detecting the 3D objects features successfully. Our work shows a proof of concept of one approach towards solving the problem, and we believe with enough training data, the same pipeline can be expanded to handle even broader set of 3D scene generation problems.

==> Sections/old_intro.tex <==
\textcolor{carmine}{control, generalized , framework, end-to-end pipeline , include both the wellness of both methods}

Recent advances in Computer Graphics have resulted in sophisticated render engines (cite few).
%Although these frameworks allow artists, animators and storytellers to design creative characters and storylines, these processes are often difficult and time-consuming.However, some render engines allow us to generate synthetic scenes using scene programs. 
Using these render engines, artists can generate scenes and videos by adding characters and objects, movement and lighting. Although these frameworks provide precision and finer control for scene generation, the process is time-consuming.  These engines works by running sophisticated program in the backend. Some engines allow users to execute these scene program to generate scene.  
%Figure ? shows a simple Blender scene program to generate a Monkey-head image.

\textit{Is it possible to automate the time-consuming task of scene generation using scene program in a controllable way?} With recent advances of Generative adversarial network~\cite{Gan} and Variational Autoencoder~\cite{vae}. we have seen a promising result in automated image and video generation from textual description. Few studies proposed Neural scene program synthesis which allows neural networks to generate programs which are rendered into images using render engines. However, a major challenge of these techniques are generalization and editability~\cite{survey}.
 
In this study, we propose a novel task - Holistic Image and Video Generation from text by leveraging scene program. Unlike prior works of directly generating final image/video from neural nets, Our proposed end-to-end framework works in two steps: First our novel architecture - Hidden2Feature encodes textual description into an abstraction of the final scene layout, second our scene program converts this abstraction into a synthetic image or video. The two-way unique pipeline provides an interpretable understanding of what our model is learning and a finer control over the scene objects via scene program.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{images/code_example.eps}
% \caption{A high resolution image of a Monkey Head generated by the two-line Blender script on the left. It is possible to generate more complicated image with more specific information. \textit{\textbf{Can we use this mechanism to generate synthetic images and videos from text?}}}
% \end{figure}
Our contributions are as follows --- 1) We propose a novel hybrid approach of both image and video generation from text which is more generalized and interpretable. Our proposed mechanism makes a bridge among automated image/video generation and existing 3D rendering engines. 2) We release a large scalable combined benchmark dataset for image and video generation from text, which will pave a way for this novel research field. 3) We show the finer control and editability of our mechanism.


% \begin{figure}[ht]
% \begin{subfigure}{.33\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{charts/image_val.pdf}
%   \caption{$M_{image}$}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.33\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{charts/video_val.pdf}
%   \caption{$M_{video}$}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.33\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{charts/comb_val.pdf}
%   \caption{$M_{full}$}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{The expected validation performance for $M_{image},~M_{video},~M_{full}$. The X and Y-axis represent epoch no. and expected validation respectively~\cite{showyourwork}}
% \label{fig:valdation_curve}
% \end{figure}

================================================

\textcolor{carmine}{control, generalized , framework, end-to-end pipeline , include both the wellness of both methods}

There are many sophisticated 3D render engines which are widely used by artists and storytellers for creative characters creation and scene rendering. While the creation involves designing new characters and animation, rendering involves making the final scene by including the characters, adding animation and other post-processing to form a story plot. The main advantage of these engines is the ability to achieve detailed features and control. However, both of these tasks are time consuming and require manual intervention. With recent advances of Generative adversarial network(GAN) and Variational Autoencoder(VAE), we have seen a promising improvement in automated image and video generation, character creation. However the concept of automated scene rendering is relatively unexplored. Unlike automated generation, automated scene rendering is related to automated creation of the final layout with predefined characters, textures and animation. Such a task is more applicable over automated generation, when we wish to have specialized characters but automate the process of scene rendering with a given story plot. A relevant example is the 3D animated movies where we see a wide range of characters varying from movies to movies, but some actions are common for all (singing, dancing, running, etc.), thus follow a learnable pattern.

At the heart of 3D rendering engines, are sophisticated algorithms in the backend. Some engines allow users to execute scene programs as API to generate scenes. Is it possible to automate the time-consuming task of scene rendering using scene program in a controllable way?

In this study, we propose a novel task - Holistic Image and Video rendering from text by leveraging scene program. Our end-to-end framework works in two steps: First our novel network architecture - Hidden2Feature encodes textual description into an abstraction of the final scene layout, second our scene program renders this abstraction into a synthetic image or video. The two-way unique pipeline provides an interpretable understanding of what our model is learning and a finer control over the scene objects via scene program.we provide a quantitative analysis on how our model adopts even on novel scene description and enables us include new, unseen scene objects at inference.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{images/code_example.eps}
% \caption{A high resolution image of a Monkey Head generated by the two-line Blender script on the left. It is possible to generate more complicated image with more specific information. \textit{\textbf{Can we use this mechanism to generate synthetic images and videos from text?}}}
% \end{figure}
Our contributions are as follows --- 1) We propose a novel hybrid approach of both image and video generation from text which is more generalized and interpretable. Our proposed mechanism makes a bridge among automated image/video generation and existing 3D rendering engines. 2) We release a large scalable combined benchmark dataset for image and video generation from text, which will pave a way for this novel research field. 3) We show the finer control and editability of our mechanism.
